B-fields In STar-forming Region Observations (BISTRO): Dual-Wavelength Constraints on Size-Dependent Grain Alignment in Star-Forming Regions

We compared 450 and 850 $\mu$m POL-2 observations from the James Clerk Maxwell Telescope at $12.6''$ resolution. The median absolute difference in polarization angle between bands is $6.7^\circ$ across 21 regions. For total intensity $I\propto\nu^\alpha$ and polarized intensity $PI\propto\nu^\gamma$, 24-27 of 35 regions have $\gamma<\alpha$, allowing for $3\sigma$ limits on weak polarized intensities. The median $\gamma-\alpha$ is $-0.51$, ranging from $-0.57$ to $-0.45$ under these limits. The ratio of polarization fractions is $P_{450}/P_{850}=0.69\pm0.02_{\rm sys}\pm0.03_{\rm stat}$, with no detected dependence on the angle difference. We suggest that the dependence of alignment on grain size offers the simplest explanation of these findings. For optically thin components sharing a polarization angle and opacity law, temperature mixing reproduces the median $-0.51$ only if the warm dust is polarized less efficiently than the cold dust. If the cold dust is at 10 K or warmer and the warm dust at 40 K or cooler, the median requires a ratio of warm to cold effective polarization efficiencies $r\lesssim0.18$. We tested mixtures with opacity index $\beta=2$ in four fields against Herschel dust temperatures and Green Bank Ammonia Survey kinetic temperatures. We assumed equal gas and dust temperatures, ammonia tracing cold gas, and model ranges of 3-20 K for cold dust and 25-40 K for warm dust carrying at most half the mass. Mixtures matching both temperatures cannot reproduce $\gamma-\alpha$ within $1\sigma$ in three fields, including OMC 2 tentatively, even for $r=0$. Allowing warm dust at 10-100 K and up to 95% of the mass permits solutions only for $r\leq0.041$. To explain these three fields by temperature mixing, we need wider model ranges and a very strong contrast in polarization efficiency. The origin of this contrast remains undetermined.

==> xref_frozen_S1_pasj.tex <==
\makeatletter
\newlabel{S2-app:S2_survey_fields}{{6}{80}{}{section.\theH@article .6}{}}
\newlabel{S2-app:distance}{{5}{79}{}{section.\theH@article .5}{}}
\newlabel{S2-eq:planck_correction}{{9}{33}{}{equation.\theH@article .9}{}}
\newlabel{S2-fig:env_ladder}{{11}{47}{}{figure.\theH@article .11}{}}
\newlabel{S2-sec:S2_results}{{3}{12}{}{section.\theH@article .3}{}}
\newlabel{S2-ss:S2_EnvStrat}{{3.5}{42}{}{subsection.\theH@article .5}{}}
\newlabel{S2-ss:S2_P_ratio}{{3.3}{22}{}{subsection.\theH@article .3}{}}
\newlabel{S2-ss:S2_SP}{{3.2}{19}{}{subsection.\theH@article .2}{}}
\newlabel{S2-ss:S2_SpIdx}{{3.4}{32}{}{subsection.\theH@article .4}{}}
\newlabel{S2-sss:S2_source_aware_correlation}{{3.6.11}{61}{}{subsubsection.\theH@article .11}{}}
\newlabel{S2-sss:S_definition}{{3.1.1}{14}{}{subsubsection.\theH@article .1}{}}
\newlabel{S2-sss:SpIdxFramework}{{3.4.1}{32}{}{subsubsection.\theH@article .1}{}}
\newlabel{S2-sss:SpIdx_Global}{{3.4.3}{34}{}{subsubsection.\theH@article .3}{}}
\newlabel{S2-tab:surv}{{19}{81}{}{table.\theH@article .19}{}}
\newlabel{S2-tbl:S2_F4F6_master}{{2}{8}{}{table.\theH@article .2}{}}
\newlabel{S2-tbl:S2_dependency}{{3}{13}{}{table.\theH@article .3}{}}
\newlabel{S2-tbl:SpIdx_Global}{{7}{40}{}{table.\theH@article .7}{}}
\newlabel{S2-tbl:env_4metric}{{8}{50}{}{table.\theH@article .8}{}}
\newlabel{S2-tbl:influential_source_policy}{{11}{64}{}{table.\theH@article .11}{}}
\newlabel{T-app:mas_debias}{{10}{72}{}{section.\theH@article .10}{}}
\newlabel{T-app:pca_mosaicking}{{7.2}{67}{}{subsection.\theH@article .2}{}}
\newlabel{T-eq:planck_correction}{{8}{10}{}{equation.\theH@article .8}{}}
\newlabel{T-eq:precision_floors}{{57}{53}{}{equation.\theH@article .57}{}}
\newlabel{T-sec:precisionfloor}{{4.2}{53}{}{subsection.\theH@article .2}{}}
\newlabel{T-sec:techresults}{{3}{7}{}{section.\theH@article .3}{}}
\newlabel{T-sec:uncertainty}{{4.1}{50}{}{subsection.\theH@article .1}{}}
\newlabel{T-ss:beamval}{{3.5}{45}{}{subsection.\theH@article .5}{}}
\newlabel{T-ss:flux}{{3.1}{7}{}{subsection.\theH@article .1}{}}
\newlabel{T-ss:noiseI}{{3.2}{11}{}{subsection.\theH@article .2}{}}
\newlabel{T-ss:noisemodel}{{3.3}{24}{}{subsection.\theH@article .3}{}}
\newlabel{T-ss:offset}{{3.4}{32}{}{subsection.\theH@article .4}{}}
\newlabel{T-ss:spidx_snrbias}{{3.3.7}{31}{}{subsubsection.\theH@article .7}{}}
\newlabel{T-ss:spidx_snrbias_sens}{{3.3.9}{31}{}{subsubsection.\theH@article .9}{}}
\newlabel{T-tbl:T_sample_inventory}{{2}{6}{}{table.\theH@article .2}{}}
\newlabel{T-tbl:systematics}{{7}{52}{}{table.\theH@article .7}{}}
\makeatother

